FeatNavigator: Automatic Feature Augmentation on Tabular Data

Data-centric AI focuses on understanding and utilizing high-quality, relevant data in training machine learning (ML) models, thereby increasing the likelihood of producing accurate and useful results. Automatic feature augmentation, aiming to augment the initial base table with useful features from other tables, is critical in data preparation as it improves model performance, robustness, and generalizability. While recent works have investigated automatic feature augmentation, most of them have limited capabilities in utilizing all useful features as many of them are in candidate tables not directly joinable with the base table. Worse yet, with numerous join paths leading to these distant features, existing solutions fail to fully exploit them within a reasonable compute budget. We present FeatNavigator, an effective and efficient framework that explores and integrates high-quality features in relational tables for ML models. FeatNavigator evaluates a feature from two aspects: (1) the intrinsic value of a feature towards an ML task (i.e., feature importance) and (2) the efficacy of a join path connecting the feature to the base table (i.e., integration quality). FeatNavigator strategically selects a small set of available features and their corresponding join paths to train a feature importance estimation model and an integration quality prediction model. Furthermore, FeatNavigator's search algorithm exploits both estimated feature importance and integration quality to identify the optimized feature augmentation plan. Our experimental results show that FeatNavigator outperforms state-of-the-art solutions on five public datasets by up to 40.1% in ML model performance.

==> sections/6_exp_old.tex <==
\section{Experimental Evaluation}
\label{sec:exp}

\subsection{Experimental Setup}
\label{sec:exp:setup}

\para{Data Sets.} We evaluate \method\ using three real-world data sets for classification and regression tasks. All three datasets are composed based on base tables provided by Kaggle and the DARPA Data Driven Discovery of Models (D3M)\footnote{\url{https://datadrivendiscovery.org/about-d3m/}}. Given a base table, we searched open source datasets for joinable tables using NYU Auctus~\cite{auctus} to identify candidate tables to augment.

\begin{itemize}[leftmargin=*]
    \item \textbf{School}. This is a classification dataset commonly used in baselines~\cite{arda,autof,metam}. The target prediction is school performance on a standardized test based on student attributes, course attributes and other historical surveys. We identified \textcolor{blue}{1,065} candidate features for augmentation.
    \item \textbf{DonorsChoose\footnote{\url{https://www.kaggle.com/c/donorschoose-application-screening}}}. This is also a classification dataset obtained from Kaggle. The target prediction is whether DonorsChoose proposal was accepted. We identified \textcolor{blue}{122} candidate features for augmentation.
    \item \textbf{Fraud Detection\footnote{\url{https://www.kaggle.com/competitions/ieee-fraud-detection}}}. This classification dataset from Kaggle consists of over 800 \jiaming{we don't have so many because we dropped many useless columns in the base table at the beginning.} candidate features. The task is to predict whether an online transaction is fraudulent.
\end{itemize}
\chuan{do we have any dataset for regression tasks?}
\jiaming{no by now}

Note that tables from Kaggle are typically wide consisting many features already integrated with base tables. Hence we normalize these wide tables and consequently generate candidate tables with features more than 1-hop away from the original base tables. Table~\ref{tab:dataset_stat} provides the basic information about the three datasets. The numbers of 1-hop and 2-hop features are reported as well.

\input{tables/dataset}

\para{Baselines.} We compared \method with a variety of baselines, including heuristic-based solutions such as Deep Feature Synthesis and ARDA as well as machine learning-based solutions such as AutoFeature and METAM. 

\begin{itemize}[leftmargin=*]
    \item Deep Feature Synthesis (DFS)~\cite{dfs} is a pioneer work that automatically generates features for relational datasets. DFS utilizes relationships in the data to a base field, and then sequentially applies mathematical functions along that path to create the final feature.
    \item ARDA~\cite{arda} is a feature augmentation system, which employs a variety of heuristics to select top-k tables to join and uses a random injection-based feature augmentation to search candidate feature subsets.
    \item AutoFeature~\cite{autof} is a reinforcement learning based framework to augment the features following an exploration-exploitation strategy over the search space of candidate tables (features).    
    \item METAM~\cite{metam} is a goal-oriented framework that queries the downstream task with a candidate dataset, forming a feedback loop that automatically steers the discovery and augmentation process.
\end{itemize}

\para{Evaluation Metrics.} Since we have two different types of tasks, i.e., classification and regression, we use Area Under Curve (AUC) and Mean Squared Error (MSE) for these two tasks, respectively.
(1) AUC is a commonly used metric for classification tasks to assess the discriminative power of the predictive classification model. AUC is the area under the ROC curve. Thus, the value of AUC is between [0,1]. ROC curve is the plot of the rate of true positives (TPR, computed by TPR = TP/(TP+FN)) versus the rate of false positives (FPR, computed by FPR = FP/(TN+FP)) at different probability cutoffs. The higher the AUC score, the better the model.
(2) MSE is often used to evaluate the performance of the regression model. MSE takes the distances from the normalized points of ground truth (y) to the regression line ($y_{\textit{predict}}$) and squaring them, i.e., \(MSE = \frac{1}{n}\sum_{i=1}^{n}(y-y_{\textit{predict}})^2\). The lower the MSE, the better the prediction.


\subsection{Main Experiment}
\label{sec:exp:main}

In the end-to-end evaluation, our goal is to show how \method performs compared against the above mentioned baselines in feature augmentation. We apply \textcolor{blue}{xxx} as the given budget to all methods.

The results shown in Table.~\ref{tab.main_exp}


\begin{table*}[htbp]
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
\toprule
     \multirow{2}{*}{Dataset} & \multirow{2}{*}{Metrics} & \multirow{2}{*}{Feature Budget} & \multicolumn{5}{c}{Method}\\
     \cline{4-8}
     &  &  & DFS & iARDA & AutoFeature & METAM & \method \\
    \hline
    \multirow{3}{*}{DonorChoose} & \multirow{3}{*}{Accuracy} & 1 & 0.655 & 0.856 & 0.708 & 0.656 & 0.822\\
     &  & 5 & 0.820 & 0.890 & 0.852 & 0.659 & 0.954\\
     &  & 10 \jiaming{provide path length distribution} & 0.858 & 0.901 & 0.961 \jiaming{double check} & 0.871 & 0.961\\
     \hline
     \hline
    \multirow{3}{*}{Fraud Detection} & \multirow{3}{*}{F1}  & 1 & 0.068 & 0.131 & 0.108 & 0.437 & 0.353 \\
     &  & 5 & 0.070 & 0.151 & 0.109 & 0.464 & 0.493\\
     &  & 10 & 0.084 & 0.155 & 0.109 & 0.464 & 0.540\\
     \hline
     \hline
     \multirow{3}{*}{School} & \multirow{3}{*}{Accuracy} & 1 & 0.704 & 0.697 & 0.708 & 0.790 & 0.823\\
     & & 5 & 0.700 & 0.808 & 0.704 & 0.801 & 0.891\\
     & & 10 & 0.692 & 0.794 & 0.723 & 0.816 & 0.880\\
 \bottomrule
\end{tabular}
\caption{Main Experiment Result}
\label{tab.main_exp}
\end{table*}


\begin{comment}
\begin{figure*}
  \centering
  \includegraphics[width=\linewidth]{figures/main_exp.pdf}
  \caption{Main Experiment Result}
  \label{fig:main_exp}
\end{figure*}
\end{comment}


\subsection{Ablation Study}
\label{sec:exp:ablation}

To better understand how our key designs of \method benefit the overall performance feature exploration and exploitation, we conduct an extensive ablation study to evaluate the performance of \method's individual components and their variants.

\begin{comment}
\begin{figure}
  \centering
  \includegraphics[width=\linewidth]{figures/exp.iq.pdf}
  \caption{IQ Experiment Result \jiaming{need update}}
  \label{fig:iq_exp}
\end{figure}
\end{comment}

\subsubsection{Effectiveness of \method's Integration Quality Model.}

\para{Effectiveness of \method's Integration Quality Model.} 
In this experiment, we do the following over 3 datasets.\\
(1) Baseline: random, quantile points in range, selectivity multiplication, and ?\\
(2) Vary training budget\\
(3) Measure MSE

The results are shown in Table.~\ref{tab.iq_budget_exp}.
\input{tables/ablation:iq}


















\subsubsection{Effectiveness of \method's Feature Importance Estimator.}
\para{Effectiveness of \method's Feature Importance Estimator.}
In this experiment, we do the following over 3 datasets.\\
\jiaming{evaluating cluster quality}

(1) Vary training $budget=B$ 

(2) MAE($estimated\_IQ$, $ground\_truth\_IQ$)

(3) Baseline: random, centroid-based, top-k centroids, top-k distance-based coverage?
\begin{enumerate}
\item \textbf{Random Sampling:} Randomly choosing \textit{B} destination features for estimating FI (Feature Importance) in data points. Ensuring that each cluster contains at least one data point.

\item \textbf{Top Centroids Approach:} Allocating budgets uniformly across clusters. Within each cluster, selecting the top central data points.

\item \textbf{Top Cover Strategy:} Equally distributing budgets across clusters. The objective within each cluster is to identify points that minimize the \textbf{coverage radius}. Given the NP-hard nature of this problem \cite{}, we employ a greedy approach: iteratively selecting unchosen points with the maximum distance from the closest selected point.

\end{enumerate}





The results are shown in Tab.~\ref{tab.fi_exp}.


\input{tables/ablation:fi}




\subsubsection{Effectiveness and Efficiency of \method's Search Algorithm.}
\para{Effectiveness and Efficiency of \method's Search Algorithm.}
In this experiment, we do the following over 3 datasets.\\
We vary the number of feature to augment and compare our search algorithm with other baseline search algorithms. The search time and downstream performance (utility gain) are for comparision. The baselines are:
\begin{enumerate}
\item \textbf{Exhausive:} Use BFS to exhaustively find out and estimate all possible destination features/join paths.

\item \textbf{Greedy:} Greedily use features with highest estimated FI for candidate features. For each candidate feature, use the path with the fewest number of joins. If more than one join paths are in the shortest length, use the one with the highest estimated IQ.
\end{enumerate}


The results are shown in Fig.~\ref{tab.search_exp}. The results show that: (1) our method is more efficient that Exhaustive while having a comparable downstream utility gain; (2) our method is much more effective that the greedy baseline.
\input{tables/ablation:search}







\subsubsection{End-to-End Latency}
% \para{End-to-End Latency}

In this experiment, we set up a utility score lower bound for each task, and vary the budget for each method to satisfy the lower bound. The end-to-end processing time is for comparision. If the method cannot achieve the goal with in \jiaming{xxx}, we will report the best possible score within the time limitation.
\input{tables/ablation:e2e}





